Understanding the Generalization Benefit of Normalization Layers: Sharpness Reduction

Normalization layers (e.g., Batch Normalization, Layer Normalization) were introduced to help with optimization difficulties in very deep nets, but they clearly also help generalization, even in not-so-deep nets. Motivated by the long-held belief that flatter minima lead to better generalization, this paper gives mathematical analysis and supporting experiments suggesting that normalization (together with accompanying weight-decay) encourages GD to reduce the sharpness of loss surface. Here "sharpness" is carefully defined given that the loss is scale-invariant, a known consequence of normalization. Specifically, for a fairly broad class of neural nets with normalization, our theory explains how GD with a finite learning rate enters the so-called Edge of Stability (EoS) regime, and characterizes the trajectory of GD in this regime via a continuous sharpness-reduction flow.

==> rmsdrift.tex <==

\subsection{Old Stuff}
In this section, we give a proof sketch for \Cref{thm:fullspace-main},
the main theorem for the case of full-space optimization.


Fix $T > 0$ and a RMSdrift flow $\vzeta: [0, T] \to \manGa$ starting from $\vzeta_0$.

Proof idea: show that RMSprop is a RMSdrift process (defined below). Then we establish a general equivalence between the discrete RMSdrift process and the continuous 
RMSdrift flow when $\eta \to 0$.

Let $\manGa' := \bigcup_{t \in [0, T]} \{ \vphi \in \manGa : \normtwosm{\vphi - \vzeta(t)} \le r \}$
be a submanifold of $\manGa$,
where $r > 0$ is a sufficiently small constant so that the boundaries of manifolds $\manGa$ and $\manGa'$ do not intersect.
Then $\manGa'$ is compact.

For any local minimizer 
$\vtheta \in \manGa'$,
we define $\gamma(\vtheta) := \frac{1}{\lamH_1(\vtheta)} \min\left\{\lamH_1(\vtheta) -
\lamH_2(\vtheta), \lamH_{D-\DGa}(\vtheta)\right\} $ to be the
relative eigenvalue gap (between $\lamH_1$ and $\lamH_2$, or between $\lamH_{D- \DGa}$ and $0$).

By the compactness of $\manGa'$ and \Cref{ass:man,ass:rank,ass:topeigen},
the minimum relative eigenvalue gap $\gamin := \inf_{\vtheta \in \manGa'} \{\gamma(\vtheta)\}$ over $\manGa'$ is non-zero.

For all $\vtheta \in \UGa$, define $\Phi(\vtheta)$ to be the convergence point of the gradient flow
starting from $\vtheta$. By \Cref{ass:man}, we know that $\Phi(\vtheta) \in \manGa$.
It has been proved by \kaifeng{XXX} that $\Phi$ is $\contC^2$-smooth on $\UGa$.


\subsubsection{RMSdrift Process}

\begin{theorem} \label{thm:rmsprop-is-rmsdrift}
  For gradient descent with $(\eta, \beta)$-RMSprop-like learning rate scheduler and $\beta = 1 - \Cb \eta^2 + O(\eta^4)$,
  define
  \begin{align*}
  \vphi_t &:= \Phi(\vtheta_t), &
  h_t &:= \frac{1}{\eta}\dotpsm{\vtheta_t - \vphi_t}{\vvH_1(\vphi_t)}, &
  w_t &:= \frac{1}{\eta}\normtwosm{\mPw_t (\vtheta_t - \vphi_t)}, &
  u_t &:= \frac{1}{\eta}\left( \frac{4 \tilv_t}{\lamH_1(\vphi_t)^2} - 1 \right),
  \end{align*}
  where $\mPw_t$ is the projection matrix onto the space spanned by the eigenvectors of $\mH_t$
  corresponding to non-zero and non-top eigenvalues ($\lambda \ne 0, \lamH_1(\vphi_t)$).
  For parameters $\alpha, r \le \eta^{-o(1)}$ with $r \le O(\alpha)$, if
  $h_t \le O(r), w_t \le O(r^2 \eta)$, and $\abssm{u_t} \le O(\alpha)$, then
  \begin{align*}
    h_{t+2} &= (1 - 2 \eta u_t) h_t + \Osm{\alpha^2 r\eta^2}, \\
    w_{t+2} &\le (1-\gamma(\vphi_t))^2 w_t + O(r^2 \eta), \\
    u_{t+2} &= u_t + 4 \eta h_t^2 (2 \Cb + \normtwosm{\gradGa R(\vphi_t)}^2) - 2 \eta \Cb + \Osm{\alpha(1+r^2)\eta^2}, \\
    \vphi_{t+2} &= \vphi_t
    - 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + \Osm{\alpha r^2 \eta^3}.
  \end{align*}
\end{theorem}

Proof is deferred to \Cref{sec:connect-to-rmsdrift}.


The key ingredient of our proof is that the dynamics after the initial alignment phase
can be captured by the RMSdrift process defined below.

\begin{definition}
  A \textit{drift state} is described by a tuple $S = (h, u, \vphi)$ in the drift state space $\Sta := \Rgez \times \R \times \manGa$.
  We say that $S$ is \textit{$\alpha$-bounded} if $\max\{h, \abssm{u}\} \le \alpha$.
\end{definition}
\begin{definition}
  Given two drift states $S_0 = (h_0, u_0, \vphi_0)$, $S_2 = (h_2, u_2,
  \vphi_2)$ in the drift state space $\Sta$, we say that the transition $S_0 \to
  S_2$ is a \textit{$(C_0, \Cb, \alphamax)$-RMSdrift transition} with learning rate
  $\eta$ if, whenever $S_0$ is $\alpha$-bounded for some $1 \le \alpha \le \alphamax$, $S_2$ is close to an auxiliary state $S'_2 := (h'_2, u'_2, \vphi'_2)$ in the following sense
  \begin{align*}
    \abssm{h_2 - h'_2} &\le C_0 \alpha^2 h_0 \eta^2, \\
    \abssm{u_2 - u'_2} &\le C_0 \alpha (1 + h_0^2) \eta^2,  \\
    \normtwosm{\vphi_2 - \vphi'_2} &\le C_0 \alpha h_0^2 \eta^3,
  \end{align*}
  where $S'_2$ is defined as follows,
  \begin{align*}
    h'_2 &:= (1 - 2\eta u_0) h_0,  \\
    u'_2 &:= u_0 + 4 \eta h_0^2 (2 \Cb + \normtwosm{\gradGa R(\vphi_0)}^2) - 2\eta \Cb,  \\
    \vphi'_2 &:= \vphi_0 - 2 \eta^2 h_0^2 \gradGa R(\vphi_0).
  \end{align*}
  For a sequence of states $S_0, S_2, S_4, \dots, S_T$, we say it is a $(C_0,
  \Cb, \alphamax)$-\textit{RMSdrift process} with learning rate $\eta$ if $S_t \to S_{t+2}$ is a
  $(C_0, \Cb, \alphamax)$-RMSdrift transition with learning rate $\eta$ for all even
  numbers $0 \le t < T$.
\end{definition}

In this section, we always consider the case where $\eta \to 0$, $1 \le \alphamax \le (\tfrac{1}{\eta})^{o(1)}$ and the other
parameters $C_0 > 0$, $\Cb > 0$ are constants.
\subsubsection{Equivalence Between RMSdrift Process and Flow}

\begin{theorem}
  For any constant time $T > 0$, if $S_t$ is $\alpha$-bounded for all even numbers $t \le T / \eta^2$, then
  \[
    \vphi_t = \vzeta(\eta^2 t) + O(\alpha^2 \eta^{0.5}).
  \]
\end{theorem}

Proof is deferred to \Cref{sec:rmsdrift-proof}.


==> rmsprop-proof.tex <==

\subsubsection{Connecting to RMSdrift} \label{sec:connect-to-rmsdrift}



\begin{lemma} \label{lm:rmsprop-2-step-hw}
  Let $\alpha, r \le \eta^{-o(1)}$ with $r \le O(\alpha)$. Let $\epsilon = O(r^2)$.
  If $\normtwosm{\vx_t} \le r$, $w_t \le \epsilon$ and $\abssm{ u_t } \le \alpha$,
  then \zhiyuan{add quantifier for $t$}
  \begin{align*}
    \hath_{t+2} &= (1 - 2 \eta u_t) h_t  + \Osm{\alpha^2 r \eta^2} \\
    \hatw_{t+2} &\le (1 - \gamma)^2 w_t + O(r^2 \eta) \\
    \partial\Phi_{\vphi_t}[\hatvx_{t+2}]
    &= \partial \Phi_{\vphi_t}[\vx_t] - 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + \Osm{\alpha r^2 \eta^3} \\
    \hatu_{t+2}
    &= u_t + 8 \Cb \eta h_t^2 - 2\Cb \eta + O(\alpha(1+r^2) \eta^2).
  \end{align*}
  \kaifeng{define $\gamma$}
\end{lemma}
\begin{proof}
  By \Cref{lm:rmsprop-2-step},
  \begin{align*}
    \hatvx_{t+2} &= (\mI - \eeta_{t+1} \mH_t)(\mI - \eeta_t \mH_t) \vx_t - \vpsi_t(\vx_t) + O(\alpha r^2 \eta^3),
  \end{align*}
  Since $w_t \le \epsilon \eta^2 = O(r^2 \eta^2)$, we have $\vx_t = \eta h_t \vvH_1(\vphi_t) + O(r^2\eta^2)$.
  Then $\vpsi_t(\vx_t)$ can be approximated by
  $\vpsi_t(\vx_t) = \vpsi_t(\eta h_t \vvH_1(\vphi_t)) + O(r^2 \eta^2 \cdot r \eta)
  = \eta^2 h_t^2 \vpsi_t(\vvH_1(\vphi_t)) + O(r^3 \eta^3)$.

  Combining this with \Cref{lm:rmsprop-phi-formula} gives the projection of $\vpsi_t(\vx_t)$ onto each eigenspace:
  \begin{align*}
    \dotpsm{\vpsi_t(\vx_t)}{\vvH_1(\vphi_t)} &= 0 + O(r^3 \eta^3) = O(r^3 \eta^3), \\
    \mPw_t \vpsi_t(\vx_t) &= O(\normtwosm{\vpsi_t(\vx_t)}) = O(r^2 \eta^2), \\
    \partial \Phi_{\vphi_t}[\vpsi_t(\vx_t)] &= 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + O(r^3 \eta^3).
  \end{align*}
  
  \myparagraph{Approximation for $\hath_{t+2}$.} For $\hath_{t+2}$, we have
  \begin{align*}
    \hath_{t+2} &= \frac{1}{\eta}\left( \dotpsm{\vx_t}{(\mI - \eeta_{t+1} \mH_t)(\mI - \eeta_t \mH_t) \vvH_1(\vphi_t)} - \dotpsm{\vpsi_t(\vx_t)}{\vvH_1(\vphi_t)} + O(\alpha r^2\eta^3) \right) \\
    &= (1 - \eeta_{t+1} \lamH_1(\vphi_t)) (1 - \eeta_t \lamH_1(\vphi_t)) h_t + O(\alpha r^2 \eta^2).
  \end{align*}
  By \Cref{lm:rmsprop-2-step},
  $\eeta_{\tau} = \mu_t \cdot (1 - \tfrac{1}{2} \eta u_t) + O(\alpha^2 \eta^2)$ for both $\tau = t$ and $\tau = t+1$.
  Then by definition of $\mu_t$,
  \begin{align*}
    1 - \eeta_{\tau} \lamH_1(\vphi_t)
    &= 1 - \mu_t \cdot (1 - \tfrac{1}{2} \eta u_t) \cdot \lamH_1(\vphi_t) + O(\alpha^2 \eta^2) \\
    &= 1 - 2 \cdot (1 - \tfrac{1}{2} \eta u_t)) + O(\alpha^2 \eta^2) \\
    &= -1 + \eta u_t + O(\alpha^2 \eta^2).
  \end{align*}
  Then $(1 - \eeta_{t+1} \lamH_1(\vphi_t)) (1 - \eeta_t \lamH_1(\vphi_t)) = (-1 + \eta u_t + O(\alpha^2 \eta^2))^2 = 1 - 2 \eta u_t + O(\alpha^2 \eta^2)$,
  and thus we have
  \begin{align*}
    \hath_{t+2} = \left(1 - 2 \eta u_t + O(\alpha^2 \eta^2)\right) h_t + O(\alpha r^2 \eta^2)
    = (1 - 2 \eta u_t) h_t + O(\alpha^2 r \eta^2).
  \end{align*}

  \myparagraph{Approximation for $\hatw_{t+2}$.} To approximate $\hatw_{t+2}$, we first note that if $\vv_k$ is a $\lamH_k(\vphi_t)$-eigenvector of $\mH_t$,
  then for both $\tau = t$ and $\tau = t+1$,
  \begin{align*}
    (\mI - \eeta_\tau \mH_t) \vv_k &= \left(1 - \mu_t \cdot \left(1 - \tfrac{1}{2} \eta u_t + O(\alpha^2 \eta^2) \right) \cdot \lamH_k(\vphi_t)\right)\vv_k \\
    &= \left(1 - \frac{2}{\lamH_1(\vphi_t)} \left(1 + O(\alpha \eta) \right) \cdot \lamH_k(\vphi_t)\right)\vv_k \\
    &= \left(1 - 2 \cdot \frac{\lamH_k(\vphi_t)}{\lamH_1(\vphi_t)}\right) \vv_k + O(\alpha \eta).
  \end{align*}
  Since $\lamH_k(\vphi_t) \in [\gamma \lamH_1(\vphi_t), (1-\gamma) \lamH_1(\vphi_t)]$, we have
  $1 - 2 \cdot \frac{\lamH_k(\vphi_t)}{\lamH_1(\vphi_t)} \in [-1 + 2\gamma, 1 - 2\gamma]$.
  When $\alpha \eta$ is small, we have
  $\normtwosm{(\mI - \eeta_\tau \mH_t)\vv_k} \le 1 - \gamma$ for both $\tau = t$ and $\tau = t+1$.

  Then for $\hatw_{t+2}$ we have
  \begin{align*}
    \hatw_{t+2}
    &\le \tfrac{1}{\eta} \left(\normtwosm{ \mPw_t (\mI - \eeta_{t+1}\mH_t) (\mI -\eeta_t \mH_t) \vx_t} + \normtwosm{\mPw_t \vpsi_t(\vx_t)} + O(\alpha r^2 \eta^3)\right) \\
    &\le (1-\gamma)^2 w_t  + O(r^2 \eta).
  \end{align*}

  \myparagraph{Approximation for $\partial \Phi_{\vphi_t}[\hatvx_{t+2}]$.} 
  For $\partial \Phi_{\vphi_t}[\hatvx_{t+2}]$, we have
  \begin{align*}
    \partial \Phi_{\vphi_t}[\hatvx_{t+2}]
    = \partial \Phi_{\vphi_t}[(\mI - \eeta_{t+1} \mH_t)(\mI - \eeta_t \mH_t) \vx_t] - \partial \Phi_{\vphi_t}[\vpsi_t(\vx_t)] + O(\alpha r^2 \eta^3).
  \end{align*}
  Note that
  \Cref{lm:Phi-proj} implies that $\partial \Phi_{\vphi_t}[\vv] = \vzero$ for any $\vv \in \NGa{\vphi_t}$.
  Then we have
  \begin{align*}
    \partial \Phi_{\vphi_t}[(\mI - \eeta_{t+1} \mH_t)(\mI - \eeta_t \mH_t) \vx_t]
    &= \partial \Phi_{\vphi_t}[\vx_t] - \partial \Phi_{\vphi_t}[(\eeta_{t+1} + \eeta_t)\mH_t\vx_t] + \partial \Phi_{\vphi_t}[\eeta_{t+1} \eeta_t\mH_t^2\vx_t] \\
    &= \partial \Phi_{\vphi_t}[\vx_t].
  \end{align*}
  Combining these with $\partial \Phi_{\vphi_t}[\vpsi_t(\vx_t)] = 2\eta^2 h_t^2 \gradGa R(\vphi_t) + O(r^3 \eta^3)$ above gives
  \begin{align*}
    \partial \Phi_{\vphi_t}[\hatvx_{t+2}] &= \partial \Phi_{\vphi_t}[\vx_t] - 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + O(\alpha r^2 \eta^3).
  \end{align*}

  \myparagraph{Approximation for $\hatu_{t+2}$.} 
  By \Cref{lm:rmsprop-2-step}, we have
  \begin{align*}
    \hatu_{t+2} &= u_t + \Cb \eta \mu_t^2 \normtwosm{\mH_t \vx_t / \eta}^2 + \Cb \eta \mu_t^2 \normtwosm{\mH_t \mU_t \vx_t / \eta}^2 - 2 \Cb \eta + \Obig{\alpha(1 + r^2)\eta^2}.
  \end{align*}
  Note that
  \begin{align*}
    \normtwosm{\mH_t \vx_t / \eta}
    &= \normtwosm{\mH_t (\eta h_t \vvH_1(\vphi_t) + O(r^2 \eta^2)) / \eta} \\
    &= h_t \normtwosm{\mH_t \vvH_1(\vphi_t)} + O(r^2 \eta) \\
    &= \lamH_1(\vphi_t) h_t + O(r^2 \eta),
  \end{align*}
  where the last equality is due to $\mH_t \vvH_1(\vphi_t) = \lamH_1(\vphi_t) \vvH_1(\vphi_t)$.
  Then we can estimate the squared norm by $\normtwosm{\mH_t \vx_t / \eta}^2 = \lamH_1(\vphi_t)^2 h_t^2 + O(r^3 \eta)$.

  As $\mH_t \mU_t \vvH_1(\vphi_t) = -\lamH_1(\vphi_t) \vvH_1(\vphi_t)$, we similarly have
  $\normtwosm{\mH_t \mU_t \vx_t / \eta}^2 = \lamH_1(\vphi_t)^2 h_t^2 + O(r^3 \eta)$.

  Combining all these together gives
  \begin{align*}
    \hatu_{t+2}
    &= u_t + \Cb \eta \mu_t^2 (\lamH_1(\vphi_t)^2 h_t^2 + O(r^3 \eta)) + \Cb \eta \mu_t^2 (\lamH_1(\vphi_t)^2 h_t^2 + O(r^3 \eta)) \\
    & \quad - 2 \Cb \eta + \Obig{\alpha(1 + r^2)\eta^2} \\
    &= u_t + 8 \Cb \eta h_t^2 - 2\Cb \eta + O(\alpha(1+r^2) \eta^2).
  \end{align*}
  Hence, we have verified all the claimed approximation formulas.
\end{proof}


\begin{lemma} \label{lm:rmsprop-2-step-phi}
  In the setting of \Cref{lm:rmsprop-2-step-hw},
  \begin{align*}
    \vphi_{t+2} &= \vphi_t
    - 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + \Osm{\alpha r^2 \eta^3}. \\
    R(\vphi_{t+2}) &= R(\vphi_t)
    - 2 \eta^2 h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 + \Osm{\alpha r^2 \eta^3}.
  \end{align*}
\end{lemma}
\begin{proof}
  By Taylor expansion,
  \begin{align}
    \vphi_t &= \Phi(\vphi_t) + \partial \Phi_{\vphi_t}[\vx_t] + \frac{1}{2} \partial^2 \Phi_{\vphi_t}[\vx_t, \vx_t] + O(r^3 \eta^3). \label{eq:rmsprop-2-step-phi-taylor1} \\
    \vphi_{t+2} &= \Phi(\vphi_t) + \partial \Phi_{\vphi_t}[\hatvx_{t+2}] + \frac{1}{2} \partial^2 \Phi_{\vphi_t}[\hatvx_{t+2}, \hatvx_{t+2}] + O(r^3 \eta^3). \label{eq:rmsprop-2-step-phi-taylor2}
  \end{align}
  By definition, $\Phi(\vphi_t) = \vphi_t$. By \Cref{lm:rmsprop-2-step-hw},
  \begin{align*}
  \partial \Phi_{\vphi_t}[\hatvx_{t+2}] &= \partial \Phi_{\vphi_t}[\vx_t] - 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + \Osm{\alpha r^2 \eta^3}.
  \end{align*}
  Note that $w_t = O(r^2 \eta)$ implies that $\vx_t = \eta h_t \vvH_1(\vphi_t) + O(r^2 \eta^2)$.
  Also note that the identity
  $\partial^2 \Phi_{\vphi_t}[\vvH_1(\vphi_t), \vvH_1(\vphi_t)] = \vzero$
  holds
  by \Cref{lm:Phi-2nd-normal}. Then
  \begin{align*}
  \partial^2 \Phi_{\vphi_t}[\vx_t, \vx_t]
  &= \partial^2 \Phi_{\vphi_t}[\eta h_t \vvH_1(\vphi_t), \eta h_t \vvH_1(\vphi_t)] + O(r^3 \eta^3) \\
  &= O(r^3 \eta^3).
  \end{align*}
  Similarly, we have 
  $\partial^2 \Phi_{\vphi_t}[\hatvx_{t+2}, \hatvx_{t+2}] = O(r^3 \eta^3)$ since 
  $\hatw_{t+2} = O(r^2 \eta)$ by \Cref{lm:rmsprop-2-step-hw}.

  Now we subtract \eqref{eq:rmsprop-2-step-phi-taylor2} by \eqref{eq:rmsprop-2-step-phi-taylor1}, then
  \begin{align*}
    \vphi_{t+2} - \vphi_t
    &= \left(\partial \Phi_{\vphi_t}[\hatvx_{t+2}] - \partial \Phi_{\vphi_t}[\vx_t]\right) + \frac{1}{2} \left( \partial^2 \Phi_{\vphi_t}[\hatvx_{t+2}, \hatvx_{t+2}] - \partial^2 \Phi_{\vphi_t}[\vx_t, \vx_t] \right) + O(r^3 \eta^3) \\
    &= \left(
    - 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + \Osm{\alpha r^2 \eta^3}
    \right) + O(r^3 \eta^3) + O(r^3 \eta^3) \\
    &= - 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + \Osm{\alpha r^2 \eta^3},
  \end{align*}
  where the second line is due to \Cref{lm:rmsprop-2-step-hw}
  and
  $\partial^2 \Phi_{\vphi_t}[\vx_t, \vx_t], \partial^2 \Phi_{\vphi_t}[\hatvx_{t+2}, \hatvx_{t+2}] = O(r^3 \eta^3)$.

  For $R(\vphi_{t+2})$ we have
  \begin{align*}
    R(\vphi_{t+2}) - R(\vphi_t) 
    &= \dotpsm{\nabla R(\vphi_t)}{\vphi_{t+2} - \vphi_t} + O((r^2 \eta^2)^2) \\
    &= \dotpsm{\nabla R(\vphi_t)}{-2 \eta^2 h_t^2 \gradGa R(\vphi_t)} + \Osm{\alpha r^2 \eta^3 + r^4 \eta^4} \\
    &= -2 \eta^2 h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 + \Osm{\alpha r^2 \eta^3}.
  \end{align*}
  \kaifeng{So ...}
\end{proof}

\begin{lemma} \label{lm:rmsprop-2-step-e2e}
  In the setting of \Cref{lm:rmsprop-2-step-hw},
  \begin{align*}
    h_{t+2} &= (1 - 2 \eta u_t) h_t + \Osm{\alpha^2 r\eta^2}, \\
    w_{t+2} &\le (1-\gamma)^2 w_t + O(r^2), \\
    u_{t+2} &= u_t + 4 \eta h_t^2 (2 \Cb + \normtwosm{\gradGa R(\vphi_t)}^2) - 2 \eta \Cb + \Osm{\alpha(1+r^2)\eta^2}.
  \end{align*}
\end{lemma}
\begin{proof}
  By \Cref{lm:rmsprop-2-step-hw} and definitions of $\hath_t$ and $h_t$, $\hatw_t$ and $w_t$, $\hatu_t$ and $u_t$, we have
  \begin{align}
    \hath_{t+2} &= (1 - 2 \eta u_t) h_t  + \Obig{\alpha^2 r \eta^2} \label{eq:rmsprop-hwu-hath} \\
    \hatw_{t+2} &\le (1 - \gamma)^2 w_t + O(r^2 \eta^2) \label{eq:rmsprop-hwu-hatw} \\
    \hatu_{t+2} &= u_t + 8 \eta \Cb h_t^2 - 2 \eta \Cb + \Obig{\alpha(1+r^2)\eta^2}. \label{eq:rmsprop-hwu-hatu}
  \end{align}
  By \Cref{lm:rmsprop-2-step-phi} and definitions of $\hatvx_{t+2}$ and $\vx_{t+2}$, we have
  \begin{align*}
    \vx_{t+2} - \hatvx_{t+2} = \vphi_t - \vphi_{t+2} = 2 \eta^2 h_t^2 \gradGa R(\vphi_t) + \Osm{\alpha r^2 \eta^3}.
  \end{align*}
  And we can write $\vx_{t+2} - \hatvx_{t+2} = \vphi_t - \vphi_{t+2} = \Osm{r^2 \eta^2}$ as a loose approximation.

  \myparagraph{Approximation for $h_{t+2}$.}
  For $h_{t+2}$, we have
  \begin{align*}
    h_{t+2} - \hath_{t+2}
    &= \dotpsm{\vx_{t+2}}{\vvH_1(\vphi_{t+2})} - \dotpsm{\hatvx_{t+2}}{\vvH_1(\vphi_t)} \\
    &= \dotpsm{\vx_{t+2}}{\vvH_1(\vphi_{t+2}) - \vvH_1(\vphi_t)} + \dotpsm{\vx_{t+2} - \hatvx_{t+2}}{\vvH_1(\vphi_t)}\\
    &= O(r\eta) \cdot O(\normtwosm{\vphi_{t+2} - \vphi_t}) + 2\eta^2 h_t^2 \dotpsm{\gradGa R(\vphi_t)}{\vvH_1(\vphi_t)} + O(\alpha r^2 \eta^3) \\
    &= O(r \eta) \cdot O(r^2 \eta^2) + \Osm{\alpha r^2 \eta^3} = \Osm{\alpha r^2 \eta^3},
  \end{align*}
  where the fourth equality is due to
  $\dotpsm{\gradGa R(\vphi_t)}{\vvH_1(\vphi_t)} = 0$ and
  $\normtwosm{\vphi_{t+2} - \vphi_t} = O(r^2 \eta^2)$.
  Combining this with \eqref{eq:rmsprop-hwu-hath} proves the claimed approximation for $h_{t+2}$.

  \myparagraph{Approximation for $w_{t+2}$.}
  For $w_{t+2}$, we have
  \begin{align*}
    w_{t+2} - \hatw_{t+2}
    &= \normtwosm{\mPw_{t+2} \vx_{t+2}} - \normtwosm{\mPw_t \hatvx_{t+2}} \\
    &= \normtwo{(\mPw_t + (\mPw_{t+2} - \mPw_t)) (\hatvx_{t+2} + (\vx_{t+2} - \hatvx_{t+2}))} - \normtwosm{\mPw_t \hatvx_{t+2}} \\
    &= \normtwo{(\mPw_t + O(r^2 \eta^2)) (\hatvx_{t+2} + O(r^2\eta^2))} - \normtwosm{\mPw_t \hatvx_{t+2}} \\
    &= O(r^2 \eta^2),
  \end{align*}
  where the third equality is due to 
  $\vx_{t+2} - \hatvx_{t+2} = \vphi_t - \vphi_{t+2} = O(r^2 \eta^2)$.
  Combining this with \eqref{eq:rmsprop-hwu-hatw} proves the claimed approximation for $w_{t+2}$.

  \myparagraph{Approximation for $u_{t+2}$.}
  Now we prove the formula for $u_{t+2}$.
  Note that $\vphi_{t+2} - \vphi_t = O(r^2 \eta^2)$ implies that $\mu_{t+2} - \mu_t = O(r^2 \eta^2)$.
  Then we have
  \begin{align*}
    \eta\left(u_{t+2} - \hatu_{t+2}\right) &= (\mu_{t+2}^2 - \mu_t^2) \tilv_{t+2} \\
    &= (\mu_{t+2} - \mu_t) (2 \mu_t + O(r^2 \eta^2)) \cdot (\tfrac{1}{\mu_t^2} + O(\alpha \eta)) \\
    &= (\mu_{t+2} - \mu_t) \left( 2 \mu_t \cdot \tfrac{1}{\mu_t^2} + O(\alpha \eta) \right) \\
    &= \tfrac{2}{\mu_t}(\mu_{t+2} - \mu_t) + O(\alpha r^2 \eta^3).
  \end{align*}
  Note that $\log \mu_{t+2} - \log \mu_t = \log\left(1 + \frac{1}{\mu_t}(\mu_{t+2} - \mu_t)\right) = \tfrac{1}{\mu_t}(\mu_{t+2} - \mu_t) + O((r^2 \eta^2)^2)$. 
  By \Cref{lm:rmsprop-2-step-phi},
  \begin{align*}
    \log \mu_{t+2} - \log \mu_t = R(\vphi_t) - R(\vphi_{t+2}) = 2 \eta^2 h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 + O(\alpha r^2 \eta^3).
  \end{align*}
  Combining these together gives the following approximation for $\frac{1}{\mu_t}(\mu_{t+2} - \mu_t)$:
  \begin{align*}
    \tfrac{1}{\mu_t}(\mu_{t+2} - \mu_t) &= \log \mu_{t+2} - \log \mu_t + O(r^4 \eta^4) \\
    &= 2 \eta^2 h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 + \Osm{\alpha r^2 \eta^3} + \Osm{r^4 \eta^4} \\
    &= 2 \eta^2 h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 + \Osm{\alpha r^2 \eta^3}.
  \end{align*}
  So $\eta \left(u_{t+2} - \hatu_{t+2}\right) = 4 \eta^2 h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 + O(\alpha r^2 \eta^3)$.
  Then by \eqref{eq:rmsprop-hwu-hatu}, we have
  \begin{align*}
    u_{t+2} &= \hatu_{t+2} + 4 \eta h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 + \Osm{\alpha r^2 \eta^2} \\
    &= u_t + 8 \eta \Cb h_t^2 + 4 \eta h_t^2 \normtwosm{\gradGa R(\vphi_t)}^2 - 2 \eta \Cb + \Obig{\alpha(1+r^2)\eta^2} \\
    &= u_t + 4 \eta h_t^2 (2 \Cb + \normtwosm{\gradGa R(\vphi_t)}^2) - 2 \eta \Cb + \Osm{\alpha(1+r^2)\eta^2},
  \end{align*}
  which proves the claimed approximation for $u_{t+2}$.
\end{proof}


==> rmsprop.tex <==
\section{Main Theorems}

We study the dynamics of RMSprop when the training loss is already very small.

\subsection{Full Space Optimization}

Let $\manGa$ be a subset of $\R^D$ that consists of local minimizers of $\Loss(\vtheta)$.
We focus on the case where $\manGa$ forms a manifold, and study the dynamics near this manifold.

\begin{assumption} \label{ass:man}
  The loss function $\Loss: \R^D \to \R$ is $\contC^4$-smooth,
  and the set $\manGa$ is a $\contC^2$-smooth, $\DGa$-dimensional submanifold of $\R^D$
  for some $0 \le \DGa < D$.
  There is an open neighborhood $\UGa$ of $\manGa$ such that
  any gradient flow starting in $\UGa$ converges to a point in $\manGa$.
\end{assumption}

For $\vtheta \in \DGa$, let $\mH(\vtheta) := \nabla^2 \Loss(\vtheta)$.
We use $\lamH_k(\vtheta)$ to denote the $k$-th eigenvalue of $\mH(\vtheta)$.
Since $\manGa$ is a manifold of local minimizers,
the eigenvalues $\lamH_k(\mH(\vtheta))$ must be non-negative, and $\lamH_k(\vtheta) = 0$ for all $D - \DGa < k \le D$.
We further assume that the local minimizer manifold $\manGa$ is ``strict''
in the sense that the loss grows at least quadratically
when the parameter deviates from the manifold.
\begin{assumption} \label{ass:rank}
  For all $\vtheta \in \manGa$, $\rank(\mH(\vtheta)) = D - \DGa$. In other words, $\lamH_k(\vtheta) > 0$ for all $k \le D - \DGa$.
\end{assumption}

We also need the following regularity condition to ensure that the largest eigenvalue is unique.
\begin{assumption} \label{ass:topeigen}
  For all $\vtheta \in \manGa$, $\lamH_1(\vtheta) > \lamH_2(\vtheta)$.
\end{assumption}
\Cref{ass:rank} implies that the null space of the matrix $\mH(\vtheta)$ is equivalent to the tangent space of $\manGa$ at $\vtheta \in \manGa$. That is, $\TGa{\vtheta} = \{ \vx \in \R^D : \mH(\vtheta) \vx = \vzero \}$.
\Cref{ass:topeigen} ensures that the top eigenvalue of $\mH(\vtheta)$ is unique, and any top eigenvector is along a unique line in $\R^D$ passing through the origin.

Since $\Loss$ is $\contC^4$-smooth, $\mH$ is $\contC^2$-smooth. Under \Cref{ass:topeigen},
$\lamH_1$ is also $\contC^2$-smooth,
and we can construct $\contC^2$-smooth function $\vvH_1: \manGa \to \R^D$ so that $\vvH_1(\vtheta)$ is a unit-norm top eigenvector of $\mH(\vtheta)$ for all $\vtheta \in \manGa$.

Let $R: \manGa \to \R$ be the function $R(\vtheta) = \log \lamH_1(\vtheta)$, which is $\contC^2$-smooth. For any $\vtheta \in \manGa$, we use $\gradGa R(\vtheta)$ to denote the projection of $\nabla R(\vtheta)$ onto the tagent space $\TGa{\vtheta}$.

\begin{definition}[RMSdrift Flow]
  Given a constant $\Cb > 0$, we define the RMSdrift flow to be a trajectory $\vzeta: [0, T] \to \manGa$ that satisfies the following ODE: 
\begin{align*}
  \frac{\dd}{\dd t} \vzeta(t) = -\frac{1}{4 + \frac{2}{\Cb}\normtwosm{\gradGa R(\vzeta(t))}^2} \gradGa R(\vzeta(t)).
\end{align*}
\end{definition}

\kaifeng{explain that the RMSdrift flow is minimizing the spectral norm of Hessian.}


The effective LR is $\eeta_t = \frac{1}{\sqrt{\tilv_t}}$.
We study the dynamics at the Edge of Stability (EOS) \citep{cohen2021gradient}.
The EOS here means $\eeta_t \approx
\frac{2}{\lamH_1(\vphi)}$ for a point $\vphi \in \manGa$ that is close to
$\vtheta_t$.
Or we can write $v_t \approx \frac{1}{4}\lamH_1(\vphi)^2$.

\begin{definition}[$\alpha$-EOS state]
  For a local minimizer $\vzeta \in \manGa$ and ,
  we say that $(\vtheta, \tilv)$ is an $\alpha$-EOS state
  with respect to $\vzeta$
  if
  \begin{align}
    e^{-\alpha} \le \normtwosm{\vtheta - \vzeta} &\le \alpha \eta,
    & \abs{\tilv_t - \frac{1}{4}\lamH_1(\vzeta)^2 } &\le \alpha \eta.
  \end{align}
\end{definition}

\begin{definition}[$p$-aligned state]
  For a local minimizer $\vzeta \in \manGa$,
  we say that $(\vtheta, \tilv)$ is a $\kappa$-non-degenerate state
  with respect to $\vzeta$
  if
  \begin{align}
    \abssm{\dotpsm{\vtheta - \vzeta}{\vvH_1(\vzeta)}} \ge p \cdot \normtwosm{\vtheta - \vzeta},
  \end{align}
\end{definition}

\begin{theorem} \label{thm:rmsprop-main}
  Under \Cref{ass:man,ass:rank,ass:topeigen},
  let $\vzeta_0 \in \manGa$ be a point on the local minimizer manifold $\manGa$, and $\vzeta: [0, T] \to \manGa$ be the RMSdrift flow starting with $\vzeta(0) = \vzeta_0$.
  Consider the case where we run gradient descent with $(\eta, \beta)$-RMSprop-like learning rate scheduler,
  where $\eta > 0$ is the base learning rate and $\beta = 1 - \Cb \eta^2 + O(\eta^4)$ is the discount factor with $\Cb > 0$ being a constant.
  Let $\alpha_0 > 0$ be a parameter that scales as $\alpha_0 \le \eta^{-o(1)}$ when $\eta \to 0$.
  For all $\alpha_0$-EOS and $\Omega(\eta^{0.99})$-aligned initial state $(\vtheta_0, \tilv_0)$ with respect to $\vzeta_0$,
  and for every integer $0 \le t \le T / \eta^2$,
  we have the following bound between $\vtheta_t$ and the RMSdrift flow,
  \begin{equation}
    \vtheta_t = \vzeta(t \eta^2) + O(\eta^{0.5 - o(1)}).
  \end{equation}
\end{theorem}

\kaifeng{Explain that this means RMSprop tends to minimize the spectral norm of Hessian}

\begin{corollary}
  In the setting of \Cref{thm:rmsprop-main}, the same statement is true for Scalar RMSprop when $\beta = 1 - \Cb \eta^2$ for some constant $\Cb > 0$.
\end{corollary}


\subsection{Spherical Optimization}

\begin{assumption} \label{ass:sph-man}
  The loss function $\Loss$ is scale-invariant and $\contC^4$-smooth,
  and the set $\manGa$ is an open, $\contC^2$-smooth, $(\DGa-1)$-dimensional submanifold
  $\sphS^{D-1} := \{ \vtheta \in \R^D : \normtwosm{\vtheta} = 1\}$ for some $1 \le \DGa < D$.
\end{assumption}

\begin{theorem}
  Under \Cref{ass:sph-man,ass:rank,ass:topeigen}, the same statement as in \Cref{thm:rmsprop-main} holds for projected gradient descent
  with any RMSprop-like learning rate scheduler.
\end{theorem}

==> scalar-rmsprop-thm.tex <==
\section{Main Results for Scalar RMSprop} \label{sec:scalar-rmsprop-main}

As mentioned in \Cref{sec:proof-idea},
a key step in our analysis is to show the oscillation and periodic behaviors
of the effective learning rates.
But these behaviors can show up in other algorithms
besides \GDWD on scale-invariant loss.
In this section, we generalize our main theorem \Cref{thm:gdwd-main} to RMSprop
with scalar learning rate, which we call \textit{Scalar RMSprop}.

The usual RMSprop algorithm maintains a vector $\vv_t$ storing the moving
average of the squared gradients for every coordinate, i.e., $\vv_{t+1} \gets \beta \vv_t + (1-\beta) (\nabla \Loss(\vtheta_t))^{\odot 2}$,
where $\vg^{\odot 2}$ stands for the vector obtained by squaring $\vg$ coordinatewise.
When updating the training parameter, RMSprop divides the usual GD update by the square root of the moving average coordinatewise,
i.e., $\vtheta_{t+1} \gets \vtheta_t - \frac{\eta}{\sqrt{\vv_{t+1} + \epsilon}} \odot \nabla \Loss(\vtheta_t)$,
where 
$\epsilon$ is a small constant to avoid division by zero. 
Here all the addition, division, square root operations are coordinatewise,
and $\odot$ stands for coordinatewise multiplication.

Now we consider a variant of RMSprop, called \textit{Scalar RMSprop}, where
the moving average $v_t$ is maintained as a scalar storing the moving average of the squared norm of gradients,
rather than a vector that stores the moving averages separately for each coordinate.

\begin{definition}[Scalar RMSprop] \label{def:scalar-rms-std}
\textit{Scalar RMSprop} is an iterative method with
hyperparameters $\eta, \beta$.
The update rule is $\vtheta_{t+1} \gets \vtheta_t - \frac{\eta}{\sqrt{v_t}} \nabla \Loss(\vtheta_t)$,
$v_{t+1} \gets \beta v_t + (1-\beta) \normtwosm{\nabla \Loss(\vtheta_t)}^2$.
\end{definition}
\kaifeng{add related works}
Similar to \GDWD on scale-invariant function, 
we can define the \textit{effective learning rate}
to be the learning rate that is actually used for update in a specific step.
Here we define 
it to be $\eeta_t := \frac{\eta}{\sqrt{v_t}}$.

\begin{assumption} \label{ass:full-man}
  The loss function $\Loss: \R^D \to \R$ is $\contC^4$-smooth.
  $\manGa$ is a $\contC^2$-smooth, $\DGa$-dimensional submanifold of $\sphS^{D-1}$
  for some $0 \le \DGa \le D$, where every $\vtheta \in \manGa$ is a local minimizer of $\Loss$ on $\R^{D}$
  and $\rank(\mH(\vtheta)) = D - \DGa$.
\end{assumption}


We focus on the case where $\beta = \Cb \eta^2$
for some constant $\Cb$.
Our analysis shows that if Scalar RMSprop
moves close to $\manGa$ and enter the EoS regime (meaning that $\eeta_t \approx \lambda_1(\nabla^2 \Loss)$ locally)
then it follows a sharpness-reduction flow on $\manGa$ described by the following ODE,
\begin{equation}
    \vzeta(0) = \vzeta_0 \in \manGa, \qquad \frac{\dd}{\dd \tau} \vzeta(\tau) = -\frac{\gradGa \log \lamH_1(\vzeta(\tau))}{4 + \frac{2}{\Cb}\normtwosm{\gradGa \log \lamH_1(\vzeta(\tau))}^2},
    \label{eq:rmsprop-zeta}
\end{equation}
\begin{theorem} \label{thm:scalar-rmsprop-main}
  Under \Cref{ass:full-man,ass:topeigen},
  let $\vzeta_0 \in \manGa$ be a point on the local minimizer manifold.
  Consider Scalar RMSprop with learning rate $\eta > 0$ and decay rate $\beta = \Cb \eta^2$, where $\Cb$ is some constant.
  Suppose that $(\vtheta_0, v_0)$ are initialized separately as follows:
  \begin{enumerate}
    \item $\vtheta_0 = \vzeta_0 + \vxi$,
    where $\vxi \sim \Normal(\vzero, \sigma_0^2 \mI / D)$ is Gaussian noise
    with $\sigma_0 \in [\exp(-\eta^{-o(1)}), \eta^{1-o(1)}]$;
    \item $v_0$ is chosen so that $\eeta_0 := \frac{\eta}{\sqrt{v_t}}$
    satisfies $\abs{\eeta_0 - \frac{2}{\lamH_1(\vzeta_0)}} \le \eta^{1-o(1)}$.
  \end{enumerate}
  Then with probability $1 - O(\eta)$,
  the trajectory of $\vtheta_t$ is close to a sharpness-reduction flow $\vzeta: [0, T] \to \manGa$
  that starts from $\vzeta_0$ and evolves as the ODE \eqref{eq:main-zeta} (if solution exists),
  in the sense that $\normtwosm{\vtheta_t - \vzeta(t \eta^2)} = O(\eta^{1/2 - o(1)})$ for all $0 \le t \le T / \ieta$.
\end{theorem}
